Flip-OFDM for Unipolar Communication Systems

Unipolar communications systems can transmit information using only real and positive signals. This includes a variety of physical channels ranging from optical (fiber or free-space), to RF wireless using amplitude modulation with non-coherent reception, to baseband single wire communications. Unipolar OFDM techniques enable to efficiently compensate frequency selective distortion in the unipolar communication systems. One of the leading examples of unipolar OFDM is asymmetric clipped optical OFDM (ACO-OFDM) originally proposed for optical communications. Flip-OFDM is an alternative approach that was proposed in a patent, but its performance and full potentials have never been investigated in the literature. In this paper, we first compare Flip-OFDM and ACO-OFDM, and show that both techniques have the same performance but different complexities (Flip-OFDM offers 50% saving). We then propose a new detection scheme, which enables to reduce the noise at the Flip-OFDM receiver by almost 3dB. The analytical performance of the noise filtering schemes is supported by the simulation results.

==> Makefile <==

BIBDIR=../../bibs
TMPDIR=~/tmp

# Pattern rules:
%.eps : %.tiff
	tiff2ps $< > $@

all: two-stage-adaptive-cac.pdf two-stage-adaptive-cac.ps 

# images when they are converted to PDF. Without this switch, 
# EPS graphics in the final PDF look very fuzzy, especially when viewed with 
# a projector.
two-stage-adaptive-cac.pdf: two-stage-adaptive-cac.ps
	ps2pdf -dPDFsettings=/prepress two-stage-adaptive-cac.ps

# The -G0 parameter passed to dvips is used to get around a bug 
# in GhostScript which converts the "f" character to a pound 
# sign in the final PDF.
two-stage-adaptive-cac.ps: two-stage-adaptive-cac.dvi
	dvips -t a4 -Ppdf -G0 -f <two-stage-adaptive-cac.dvi >two-stage-adaptive-cac.ps

two-stage-adaptive-cac.dvi: two-stage-adaptive-cac.tex \
			  $(BIBDIR)/cac.bib \
			  $(BIBDIR)/abbrev.bib \
			  $(BIBDIR)/crossref.bib 
	latex two-stage-adaptive-cac
	bibtex two-stage-adaptive-cac
	latex two-stage-adaptive-cac
	latex two-stage-adaptive-cac


.PHONY: spell
spell : two-stage-adaptive-cac.tex two-stage-adaptive-cac.dict
	cat two-stage-adaptive-cac.tex | ispell  -l -t -a -p two-stage-adaptive-cac.dict | sort | uniq

.PHONY: clean
clean :
	rm -f *.dvi *.log *.aux *.bbl *.blg *.toc
	rm -f *~











